SplatFlow: Multi-View Rectified Flow Model for 3D Gaussian Splatting Synthesis

Text-based generation and editing of 3D scenes hold significant potential for streamlining content creation through intuitive user interactions. While recent advances leverage 3D Gaussian Splatting (3DGS) for high-fidelity and real-time rendering, existing methods are often specialized and task-focused, lacking a unified framework for both generation and editing. In this paper, we introduce SplatFlow, a comprehensive framework that addresses this gap by enabling direct 3DGS generation and editing. SplatFlow comprises two main components: a multi-view rectified flow (RF) model and a Gaussian Splatting Decoder (GSDecoder). The multi-view RF model operates in latent space, generating multi-view images, depths, and camera poses simultaneously, conditioned on text prompts, thus addressing challenges like diverse scene scales and complex camera trajectories in real-world settings. Then, the GSDecoder efficiently translates these latent outputs into 3DGS representations through a feed-forward 3DGS method. Leveraging training-free inversion and inpainting techniques, SplatFlow enables seamless 3DGS editing and supports a broad range of 3D tasks-including object editing, novel view synthesis, and camera pose estimation-within a unified framework without requiring additional complex pipelines. We validate SplatFlow's capabilities on the MVImgNet and DL3DV-7K datasets, demonstrating its versatility and effectiveness in various 3D generation, editing, and inpainting-based tasks.

==> figure/qual_result_generation.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/asset/generation_qual.pdf}
    \caption{Caption}
    \label{fig:qual_result}
\end{figure*}

==> table/inference_time.tex <==
\setlength{\columnsep}{10pt}%
\begin{wraptable}[9]{R}{0.48\linewidth}
     \centering
    \vspace{-4mm}
    \setlength\tabcolsep{3pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lc}
       \toprule
        Method   & Time \\
       \midrule
       Text2Room~\cite{wang2024prolificdreamer} & 12h \\
       DreamScene~\cite{li2024dreamscene} & 1h \\
       LucidDreamer~\cite{chung2023luciddreamer} & 5m \\
       \arrayrulecolor{gray}\midrule
       Director3D~\cite{li2024director3d} & 30s \\
       Director3D (w/ SDS++)~\cite{li2024director3d} & 5m \\
       \midrule
       \rowcolor{gray!25} \textbf{SplatFlow} & 20s \\
      \rowcolor{gray!25} \textbf{SplatFlow (w/ SDS++)} & 5m \\
       \arrayrulecolor{black}\bottomrule
    \end{tabular}
    }
    \vspace{-0.5mm}
    \vspace{\abovetabcapmargin}
    \caption{\textbf{Inference Time.}}
    \vspace{-2mm}
    \label{tab:inference_time}
\end{wraptable}


